How Quantum Agents Can Change Which Strategies Are More Complex

Whether winning blackjack or navigating busy streets, achieving desired outcomes requires agents to execute adaptive strategies, strategies where actions depend contextually on past events. In complexity science, this motivates memory as an operational quantifier of complexity: given two strategies, the more complex one demands the agent to track more about the past. Here, we show that conclusions about complexity fundamentally depend on whether agents can process and store quantum information. Thus, while classical agents might find Strategy A more complex to execute than Strategy B, quantum agents can reach the opposite conclusion. We derive sufficient conditions for such contradictory conclusions and illustrate the phenomenon across multiple scenarios. As a byproduct, our results yield an information-theoretic lower bound on the minimal memory required by any agent - classical or quantum - to execute a given strategy.

==> oharp.tex <==
\makeatletter
\newcommand{\orharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \rvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\rvectfill{%
  $\m@th\smash-\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\olharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
\mkern-7mu\smash-$}

\newcommand{\olrharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lrvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lrvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\orharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \rvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\rvectfill{%
  $\m@th\smash-\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\olharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
\mkern-7mu\smash-$}

\newcommand{\olrharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lrvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lrvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}
\makeatother
